Local near-quadratic convergence of Riemannian interior point methods

We consider Riemannian optimization problems with inequality and equality constraints and analyze a class of Riemannian interior point methods for solving them. The algorithm of interest consists of outer and inner iterations. We show that, under standard assumptions, the algorithm achieves local superlinear convergence by solving a linear system at each outer iteration, removing the need for further computations in the inner iterations. We also provide a specific update for the barrier parameter that achieves local near-quadratic convergence of the algorithm. We apply our results to the method proposed by Obara, Okuno, and Takeda (2026) and show its local superlinear and near-quadratic convergence with an analysis of the second-order stationarity. To our knowledge, this is the first algorithm for constrained optimization on Riemannian manifolds that achieves both local convergence and global convergence to a second-order stationary point. Numerical results support the theoretical analyses of the proposed methods.

==> environment/common_specific.tex <==

    %%% Specific settings
    %% general newcommand
    \newcommand{\oneline}[1]{\resizebox{\textwidth}{!}{#1}} % one line
    \newcommand{\blankline}{\vspace{\baselineskip}} % blank line
    \newcommand{\plchold}{\:\cdot\:} % placeholder
    \newcommand{\defiff}{\overser{\mathrm{def}}{\iff}} % placeholder
    \newcommand{\setR}[1][]{\mathbb{R}^{#1}}  % R (e.g., Euclidean space)
    \newcommand{\setRp}[1][]{\mathbb{R}^{#1}_{+}}  % R non negative
    \newcommand{\setRpp}[1][]{\mathbb{R}^{#1}_{++}}  % R plus
    \newcommand{\setC}[1][]{\mathbb{C}^{#1}}  % C (e.g., Complex space)
    \newcommand{\setN}[1][]{\mathbb{N}^{#1}}  % N (e.g., Natural number)
    \newcommand{\setNz}[1][]{\mathbb{N}_{0}^{#1}}  % N (e.g., Natural number with zero)
    \newcommand{\trsp}[1]{{#1}^{\top}}  % transpose
    \newcommand{\inv}[1]{{#1}^{-1}}  % inverse
    \newcommand{\adj}[1]{#1^{*}}
    %% Riemannian geometry
    \newcommand{\pt}[1][]{x_{#1}}  % point
    \newcommand{\mani}[1][M]{\mathcal{#1}}  % manifold
    \newcommand{\subsetmani}[1][U]{\mathcal{#1}}  % manifold
    \newcommand{\tanspc}[1][\pt]{T_{#1}}  % tangent space
    \newcommand{\subsettanbd}[1][S]{\mathcal{#1}}  % manifold
    \newcommand{\opensubset}[1][U]{\mathcal{#1}}  % open subset on a manifold
    \newcommand{\closedsubset}[1][P]{\mathcal{#1}}  % closed subset on a manifold
    \newcommand{\chart}[1][]{\varphi_{#1}}  % a chart on a manifold
    \newcommand{\loccoord}[1]{\overline{#1}}  % local coordinate expression

    \newcommand{\metr}[3][\pt]{\ang*{#2, #3}_{#1}}  % metric
    \newcommand{\coordmetr}[1][]{M_{#1}}  % metric under coordinates
    \newcommand{\Riemnorm}[2][\pt]{\norm*{#2}_{#1}}  % Riemannian norm
    \newcommand{\Riemdist}[3][]{\dist_{#1}\paren*{#2,#3}}  % Riemannian distance
    \newcommand{\opr}{\mathcal{A}}  % linear operator
    \newcommand{\oprtwo}{\mathcal{B}}  % linear operator 2
    \newcommand{\opnorm}[1]{\norm*{#1}_{\opstr}}  % Riemannian norm

    %% math operator
    % \DeclareMathOperator{\tr}{tr}
    % \DeclareMathOperator{\rank}{rank}
    \DeclareMathOperator{\supp}{supp}
    \DeclareMathOperator{\Det}{Det}
    \DeclareMathOperator{\diag}{diag}
    \DeclareMathOperator{\vectorize}{vec}
    \DeclareMathOperator{\poly}{poly}
    \DeclareMathOperator{\polylog}{polylog}
    \DeclareMathOperator{\Skew}{Skew}
    \DeclareMathOperator{\Sym}{Sym}
    \DeclareMathOperator{\Sympos}{\Sym_{++}}
    \DeclareMathOperator{\skewstr}{skew}
    \DeclareMathOperator{\sym}{sym}
    \DeclareMathOperator{\score}{score}
    \DeclareMathOperator{\Eig}{Eig}
    \DeclareMathOperator{\Real}{Re}
    \DeclareMathOperator{\Relerr}{Relerr}
    \DeclareMathOperator{\opstr}{op}
    \DeclareMathOperator{\strict}{str}
    \DeclareMathOperator{\Null}{Null}
    \newcommand{\restrfun}[2]{\left.#1\right|_{#2}}
    \DeclareMathOperator{\idopr}{id}  % identity operator 
    \newcommand{\id}[1][]{\idopr_{#1}}
    \newcommand{\eyemat}[1][]{I_{#1}}
    \DeclareMathOperator{\Jacob}{J}
    \newcommand{\Jacobian}[1][]{\Jacob_{#1}}
    \DeclareMathOperator{\dist}{dist}
    \DeclareMathOperator{\spanstr}{span}
    \DeclareMathOperator{\dimstr}{dim}
    \DeclareMathOperator{\Clip}{clip}
    \newcommand{\clip}[1][]{\Clip_{#1}}
    \DeclareMathOperator{\Proj}{P}
    \newcommand{\proj}[1][]{\Proj_{#1}}
    \DeclareMathOperator{\argmaxopr}{argmax}
    \DeclareMathOperator{\argminopr}{argmin}
    \newcommand{\argmin}[1][]{\underset{#1}{\argminopr}}
    \newcommand{\argmax}[1][]{\underset{#1}{\argmaxopr}}
    \newcommand{\card}[1][]{\abs*{#1}}
    \DeclareMathOperator{\minimizeopr}{minimize}
    \newcommand{\minimize}[1][]{\underset{#1}{\minimizeopr}}
    \newcommand{\subjectto}{\text{subject to}}
    
    % Riemannian geometry
    \newcommand{\Riemcxt}[2]{\nabla_{#1}#2}
    \newcommand{\covderiv}[1][]{\frac{\D}{\dd{t}}#1}
    \newcommand{\injradius}[1][]{{\rm inj}}
    \newcommand{\injradiusval}[1][]{r}
    \DeclareMathOperator{\partxpopr}{PT}  
    \newcommand{\partxp}[3][]{{\partxpopr}^{#1}_{#2\leftarrow#3}}  % parallel transport
    \newcommand{\eigval}[1][]{\lambda_{#1}} % eigen value
    
    % Riemannian optimization
    \DeclareMathOperator{\Exp}{Exp}
    \DeclareMathOperator{\Retr}{R}
    \newcommand{\retr}[1][\pt]{\Retr_{#1}}
    \newcommand{\expmap}[1][\pt]{\Exp_{#1}}
    \DeclareMathOperator{\Dopr}{D}
    \newcommand{\D}[1][]{{\Dopr}^{#1}}
    \DeclareMathOperator{\gradstropr}{grad}
    \newcommand{\gradstr}[1][]{{\gradstropr}_{#1}}
    \DeclareMathOperator{\Hessopr}{Hess}
    \newcommand{\Hess}[1][]{{\Hessopr}_{#1}}

    % Landau symbol
    \newcommand{\bigO}[1][]{\mathcal{O}\paren*{#1}}  % big O
    \newcommand{\smallO}[1][]{o\paren*{#1}}  % small O
    \newcommand{\bigomega}[1][]{\Omega\paren*{#1}}  % big omega
    \newcommand{\smallomega}[1][]{\omega\paren*{#1}}  % small omega
    \newcommand{\bigtheta}[1][]{\Theta\paren*{#1}}  % big theta
    \newcommand{\orderconstone}{\alpha}
    \newcommand{\orderconsttwo}{\beta}
    \newcommand{\ordercoeff}{c}

    % others
   \newcommand\doublecheck[1][ptblue]{\textcolor{#1}{\checked\kern-0.5em\checked}} 

    %% Algorithm
    % general
    \newcommand{\dime}{d}
    \newcommand{\ineqdime}{m}
    \newcommand{\ineqset}{\mathcal{I}}
    % \newcommand{\eqset}{\mathcal{E}}
    \newcommand{\activeineqset}{\mathcal{A}}
    \newcommand{\intvl}{I}
    \newcommand{\cid}[1][]{\simeq}  % canonical identification
    \newcommand{\RICO}{RICO}  % Riemannian inequality constrained optimization problem
    % \newcommand{\RIPM}{RIPM}  % Riemannian interior point method
    \newcommand{\IPTRM}{IPTRM}  % interior point trust region method
    \newcommand{\RIPTRM}{RIPTRM}  % Riemannian interior point trust region method
    \newcommand{\RSQO}{RSQO}  % Riemannian sequential quadratic optimization
    \newcommand{\RALM}{RALM}  % Riemannian augmented Lagrangian method
    \newcommand{\ALM}{ALM}
    \newcommand{\EPM}{EPM}
    \newcommand{\SQO}{SQO}
    \newcommand{\IPM}{IPM}
    \newcommand{\Manvio}{{\rm Manvio}}
    \newcommand{\residual}[1][]{{\rm KKT\_residual}}
    \newcommand{\secondresidual}[1][]{{\rm 2nd\text{-}order\_residual}}
    \newcommand{\posdefmanvio}[1][]{\tau_{\succ}}


    \newcommand{\Lagfun}[1][]{\mathcal{L}}  % Lagrangian for log barrier form of RICO 
    \newcommand{\criticalcone}{\mathcal{C}}  % Critical cone
    \newcommand{\weakcriticalcone}{\mathcal{C}_{{\rm w}}}  % Weak critical cone
    \newcommand{\feasirgn}{\mathcal{F}}  % Feasible region of RICO problem
    \newcommand{\strictfeasirgn}{\strict\feasirgn}  % Strict feasible region of RICO problem
    \newcommand{\SOSC}{SOSC}  % Second-order sufficient condition
    \newcommand{\SOSP}{SOSP}  % Second-order stationary point
    \newcommand{\wSOSP}{w-SOSP}  % Weak second-order stationary point
    \newcommand{\LICQ}{LICQ}  % Linear independent constraint qualification
    % \newcommand{\MFCQ}{MFCQ}  % Mangasarian-Fromovitz constraint qualification
    \newcommand{\SC}{SC}  % Strict complementary condition
    \newcommand{\KKT}{KKT}  % Karush-Kuhn-Tucker conditions
    \newcommand{\AKKT}{AKKT}  % approximate Karush-Kuhn-Tucker conditions
    \newcommand{\PAKKT}{PAKKT}  % positive approximate Karush-Kuhn-Tucker conditions
    % \newcommand{\BKKT}{BKKT}  % barrier Karush-Kuhn-Tucker conditions
    
    % functions
    \newcommand{\objfun}{f}
    \newcommand{\ineqfun}[1][]{g_{#1}}
    \newcommand{\onevec}[1][]{\bm{1}_{#1}}  % point
    \newcommand{\funone}{F}
    \newcommand{\funtwo}[1][]{\theta^{#1}}
    \newcommand{\funthr}{V}  % for vector fields 1    
    \newcommand{\funfou}{W}  % for vector fields 2
    \newcommand{\funeig}[1][]{\vartheta^{#1}}  % real-valued function 2
    \newcommand{\tanvecone}[1][\pt]{\xi_{#1}}  % tangent vector 
    \newcommand{\tanvectwo}[1][\pt]{\zeta_{#1}}  % tangent vector 
    \newcommand{\tanvecthr}[1][\pt]{\eta_{#1}}  % tangent vector 
    \newcommand{\tanvecfou}[1][\pt]{\chi_{#1}}  % tangent vector 
    \newcommand{\vecone}[1][]{v_{#1}}  % vector 
    \newcommand{\ptone}[1][]{x_{#1}}  % point
    \newcommand{\matone}[1][]{X_{#1}}  % matrix
    \newcommand{\zerovec}[1][\pt]{0_{#1}}  % zero vector
    \newcommand{\curve}[1][]{c^{#1}}  % curve
    \newcommand{\rLCone}{radially L-$C^{1}$}
    \newcommand{\rLCtwo}{radially L-$C^{2}$}
    \newcommand{\pullback}[2][]{\widehat{#2}_{#1}}
    \newcommand{\deltaRL}[1][]{\delta_{RL}^{#1}}
    \newcommand{\betaRL}[1][]{\beta_{RL}^{#1}}
    \newcommand{\deltaRLtwo}[1][]{\delta_{RL2}^{#1}}
    \newcommand{\betaRLtwo}[1][]{\beta_{RL2}^{#1}}
    \newcommand{\vecfldset}{\mathfrak{X}}
    \newcommand{\funset}{\mathfrak{F}}
    \newcommand{\ineqgradopr}[1][]{\mathcal{G}_{#1}}
    \newcommand{\coineqgradopr}[1][]{\mathcal{G}_{#1}^{\ast}}
    
    %% RIPTRM framework
    % basic
    \newcommand{\ineqidx}{i}
    \newcommand{\otriteridx}{k}
    \newcommand{\otriterpidx}{k+1}
    \newcommand{\inriteridx}{\ell}
    \newcommand{\ineqLagmult}[1][\ineqidx]{y_{#1}}  % Lagrange multipliers for inequality constraints
    \newcommand{\barrparam}[1][\otriteridx]{\mu_{#1}}  % barrier parameter
    \newcommand{\trradius}[1][\otriteridx]{\Delta_{#1}} % trust region radius
    \newcommand{\allvar}[1][]{\omega_{#1}}
    \newcommand{\barrKKTvecfld}{\Psi}  % barrier KKT vector field
    \newcommand{\IneqLagmultmat}[1][\otriteridx]{Y_{#1}}  % Diagonal matrix of Lagrange multipliers for inequality constraints
    \newcommand{\Ineqfunmat}[1][\otriteridx]{G_{#1}}  % Diagonal matrix of inequality functions    
    
    \newcommand{\forcingfun}[1][]{\varepsilon_{#1}}
    \newcommand{\forcingfungradLag}[1][]{\forcingfun[\mathcal{L}]}
    \newcommand{\forcingfunineq}[1][]{\forcingfun[I]}
    \newcommand{\forcingfunsosp}[1][]{\forcingfun[S]}
    \newcommand{\forcingfuncompl}[1][]{\forcingfun[C]}
    \newcommand{\constforcingfuncompl}[1][]{c_{C}}
    \newcommand{\constforcingfungradLag}[1][]{c_{\mathcal{L}}}

    \newcommand{\maxtrradius}{{\trradius[]}_{\max}}  % maximal trust region radius
    \newcommand{\inittrradius}{{\trradius[]}^{\rm init}}  % initial trust region radius
    \newcommand{\mininittrradius}{\inittrradius_{\min}}  % minimum initial trust region radius
    \newcommand{\finaltrradius}{{\trradius[]}^{\rm final}}  % final trust region radius
    \newcommand{\trratio}{\rho}  % trust region ratio
    % \newcommand{\trratioinriter}{\trratio^{\inriteridx}}  % 
    \newcommand{\trratioinriter}{\frac{\aredinriter}{\predinriter}} 
    \newcommand{\trratiothold}{\trratio^{\prime}}  % thereshold of trust region
    \newcommand{\contcoeff}{\gamma}  % contraction coefficient

    \newcommand{\True}{True}
    \newcommand{\False}{False}
    \newcommand{\stopcond}{COND}
    \newcommand{\seccondflag}{2ND\_ORDER}

    % Outer k-th iteration (basic)
    \newcommand{\barrparamotriter}{{\barrparam[]}_{\otriteridx}}  % barrier parameter
    \newcommand{\trradiusotriter}{{\trradius[]}_{\otriteridx}} % trust region radius
    \newcommand{\allvarotriter}{{\allvar[]}_{\otriteridx}}  % k-th all variable for RICO
    \newcommand{\ptotriter}{{\pt[]}_{\otriteridx}}  % k-th point
    \newcommand{\ineqLagmultotriter}[1][\ineqidx]{{\ineqLagmult[]}_{\otriteridx #1}}  % k-th Lagrange multipliers for inequality constraints
    \newcommand{\IneqLagmultmatotriter}{{\IneqLagmultmat[]}_{\otriteridx}}  % k-th diagonal matrix of Lagrange multipliers for inequality constraints
    \newcommand{\Ineqfunotriter}{\Ineqfunmat[]_{\otriteridx}}  % k-th diagonal matrix of inequality functions
    
    % Outer (k-1)-th iteration (basic)
    \newcommand{\barrparamotriterm}{{\barrparam[]}_{\otriteridx-1}}  % barrier parameter
    \newcommand{\allvarotriterm}{{\allvar[]}_{\otriteridx-1}}  % (k-1)-th all variable for RICO
    \newcommand{\ptotriterm}{{\pt[]}_{\otriteridx-1}}  % (k-1)-th point
    \newcommand{\ineqLagmultotriterm}[1][\ineqidx]{{\ineqLagmult[]}_{\otriteridx-1 #1}}  % (k-1)-th Lagrange multipliers for inequality constraints
    \newcommand{\IneqLagmultmatotriterm}{{\IneqLagmultmat[]}_{\otriteridx-1}}  % (k-1)-th diagonal matrix of Lagrange multipliers for inequality constraints
    \newcommand{\Ineqfunotriterm}{\Ineqfunmat[]_{\otriteridx-1}}  % (k-1)-th diagonal matrix of inequality functions
    
    % Outer (k+1)-th iteration (basic)
    \newcommand{\barrparamotriterp}{{\barrparam[]}_{\otriteridx+1}}  % barrier parameter
    \newcommand{\trradiusotriterp}{{\trradius[]}_{\otriteridx+1}} % trust region radius
    \newcommand{\allvarotriterp}{{\allvar[]}_{\otriteridx+1}}  % (k+1)-th all variable for log barrier form of RICO
    \newcommand{\ptotriterp}{{\pt[]}_{\otriteridx+1}}  % (k+1)-th point
    \newcommand{\ineqLagmultotriterp}[1][\ineqidx]{{\ineqLagmult[]}_{\otriteridx+1 #1}}  % (k+1)-th Lagrange multipliers for inequality constraints
    \newcommand{\IneqLagmultmatotriterp}{{\IneqLagmultmat[]}_{\otriteridx+1}}  % (k+1)-th diagonal matrix of Lagrange multipliers for inequality constraints
    \newcommand{\Ineqfunotriterp}{{\Ineqfunmat[]}_{\otriteridx+1}}  % (k+1)-th diagonal matrix of inequality functions
    
    % Inner l-th iteration (basic)
    \newcommand{\trradiusinriter}{{\trradius[]}^{\inriteridx}} % l-th trust region radius
    \newcommand{\allvarinriter}{{\allvar[]}^{\inriteridx}}  % l-th all variable for RICO
    \newcommand{\ptinriter}{{\pt[]}^{\inriteridx}}  % l-th point
    \newcommand{\ineqLagmultinriter}[1][\ineqidx]{{\ineqLagmult[]}^{\inriteridx}_{#1}}  % l-th Lagrange multipliers for inequality constraints
    \newcommand{\IneqLagmultmatinriter}{{\IneqLagmultmat[]}^{\inriteridx}}  % l-th diagonal matrix of Lagrange multipliers for inequality constraints
    \newcommand{\Ineqfuninriter}{{\Ineqfunmat[]}^{\inriteridx}}  % l-th diagonal matrix of inequality functions
    
    % Inner (l+1)-th iteration (basic)
    \newcommand{\trradiusinriterp}{{\trradius[]}^{\inriteridx+1}} % l-th trust region radius
    \newcommand{\allvarinriterp}{{\allvar[]}^{\inriteridx+1}}  % l+1-th all variable for RICO
    \newcommand{\ptinriterp}{{\pt[]}^{\inriteridx+1}}  % l-th point
    \newcommand{\ineqLagmultinriterp}[1][\ineqidx]{{\ineqLagmult[]}^{\inriteridx+1}_{#1}}  % l+1-th Lagrange multipliers for inequality constraints
    \newcommand{\IneqLagmultmatinriterp}{{\IneqLagmultmat[]}^{\inriteridx+1}}  % l+1-th diagonal matrix of Lagrange multipliers for inequality constraints
    \newcommand{\Ineqfuninriterp}{{\Ineqfunmat[]}^{\inriteridx+1}}  % l+1-th diagonal matrix of inequality functions
    
    % accumulation point (basic)
    \newcommand{\accumsymbol}{\ast}
    \newcommand{\allvaraccum}{{\allvar[]}^{\accumsymbol}}  % accumulation point for all variable
    \newcommand{\ptaccum}{{\pt[]}^{\accumsymbol}}  % accumlation point
    \newcommand{\ineqLagmultaccum}[1][\ineqidx]{{\ineqLagmult[]}_{#1}^{\accumsymbol}}  % accumulation point of Lagrange multipliers for inequality constraints
    \newcommand{\IneqLagmultmataccum}{{\IneqLagmultmat[]}^{\accumsymbol}}  % diagonal matrix of an accumulation point of Lagrange multipliers for inequality constraints
    \newcommand{\Ineqfunaccum}{{\Ineqfunmat[]}^{\accumsymbol}}  % diagonal matrix of inequality functions at an accumulation point

    %% RIPTRM trust region subproblem
    % model function
    \newcommand{\modelfun}[1][]{m_{#1}}
    \newcommand{\modelfuninriter}[1][]{\modelfun[#1]^{\inriteridx}}

    % quadratic and linear terms
    \newcommand{\trsquad}{H}
    \newcommand{\trslin}[1][]{{c_{#1}}}
    \newcommand{\trsquadinriter}[1][]{\trsquad_{#1}^{\inriteridx}}
    \newcommand{\trslininriter}[1][]{\trslin_{#1}^{\inriteridx}}
    \newcommand{\trsquadotriter}[1][]{\trsquad_{\otriteridx}^{#1}}
    \newcommand{\trslinotriter}[1][]{\trslin_{\otriteridx}^{#1}}
    \newcommand{\trsquadotriterp}[1][]{\trsquad_{\otriteridx+1}^{#1}}
    \newcommand{\trslinotriterp}[1][]{\trslin_{\otriteridx+1}^{#1}}

    % reduction ratio
    \newcommand{\meritfun}[1][]{P_{#1}}
    \newcommand{\ared}[1][]{{\rm ared}_{#1}}
    \newcommand{\pred}[1][]{{\rm pred}_{#1}}
    \newcommand{\aredinriter}[1][]{{\ared[#1]}^{\inriteridx}}
    \newcommand{\aredinriterp}[1][]{{\ared[#1]}^{\inriteridx+1}}
    \newcommand{\predinriter}[1][]{{\pred[#1]}^{\inriteridx}}
    \newcommand{\predinriterp}[1][]{{\pred[#1]}^{\inriteridx}}

    % search direction
    \newcommand{\dir}[1][]{d_{#1}}
    \newcommand{\dirpt}[1][]{\dir[\pt]}
    \newcommand{\dirineqLagmult}[1][\ineqidx]{\dir[{\ineqLagmult[#1]}]}
    \newcommand{\dirallvar}[1][]{\dir[{\allvar[#1]}]}
    \newcommand{\dirallvarinriter}[1][]{\dir[{\allvar[#1]^{\inriteridx}}]}
    \newcommand{\dirptinriter}[1][]{\dir[{\pt[#1]^{\inriteridx}}]}
    \newcommand{\dirineqLagmultinriter}[1][]{\dir[{\ineqLagmult[#1]^{\inriteridx}}]}

    % Cauchy step
    \newcommand{\coeffCauchy}[1][]{\tau^{#1}}
    \newcommand{\coeffCauchyoptim}{\coeffCauchy[\accumsymbol]}
    \newcommand{\dirCauchy}[1][]{\dir[#1]^{\mathrm{C}}}
    \newcommand{\dirCauchyinriter}[1][]{{\dirCauchy[{{\pt[#1]}^{\inriteridx}}]}}

    % eigenstep
    \newcommand{\diruniteigen}[1][]{s_{#1}}
    \newcommand{\diruniteigeninriter}[1][]{\diruniteigen[{\pt[#1]^{\inriteridx}}]}
    \newcommand{\epseigen}[1][]{\varepsilon_{\trsquad}}
    \newcommand{\direigen}[1][]{\dir[#1]^{\mathrm{E}}}
    \newcommand{\direigeninriter}[1][]{{\direigen[{{\pt[#1]}^{\inriteridx}}]}}
    \newcommand{\mineigval}[1][]{{\eigval[]}^{\min}_{#1}}
    \newcommand{\mineigvalinriter}{{\eigval[]}^{\inriteridx}}

    % exact step 
    \newcommand{\trsLagmult}{\nu}
    \newcommand{\trsLagmultinriter}[1][]{\trsLagmult^{\inriteridx}_{#1}}
    \newcommand{\direxact}[1][]{\dir[#1]^{\accumsymbol}}
    \newcommand{\direxactinriter}[1][]{{\direxact[{{\pt[#1]}^{\inriteridx}}]}}
    \newcommand{\direxactpt}[1][]{\dir[\pt]^{\accumsymbol}}
    \newcommand{\direxactineqLagmult}[1][]{\direxact[{{\ineqLagmult[]}_{#1}}]}
    \newcommand{\direxactallvar}[1][]{\dir[{\allvar[#1]}]^{\accumsymbol}}
    \newcommand{\direxactptotriter}[1][]{\direxact[{\ptotriter}]}
    \newcommand{\dirineqLagmultotriter}[1][]{\dir[{\ineqLagmultotriter[#1]}]}
    \newcommand{\direxactineqLagmultotriter}[1][]{\direxact[{{\ineqLagmultotriter[]}_{#1}}]}

    % Newton step
    \newcommand{\dirNewton}[1][]{{\dir[]}_{#1}^{\rm N}}
    \newcommand{\dirNewtonpt}[1][]{\dirNewton[\pt]}
    \newcommand{\dirNewtonptotriter}[1][]{\dirNewton[\ptotriter]}
    \newcommand{\dirNewtonptotriterm}[1][]{\dirNewton[\ptotriterm]}
    \newcommand{\dirNewtonineqLagmult}[1][\ineqidx]{\dirNewton[{\ineqLagmult[#1]}]}
    \newcommand{\dirNewtonineqLagmultotriter}[1][\ineqidx]{\dirNewton[{\ineqLagmultotriter[#1]}]}
    \newcommand{\dirNewtonineqLagmultotriterm}[1][\ineqidx]{\dirNewton[{\ineqLagmultotriterm[#1]}]}
    \newcommand{\dirNewtonallvar}[1][\ineqidx]{\dirNewton[{\allvar[]}]}
    \newcommand{\dirNewtonallvarotriter}[1][\ineqidx]{\dirNewton[{\allvarotriter}]}
    \newcommand{\dirNewtonallvarotriterm}[1][\ineqidx]{\dirNewton[{\allvarotriterm}]}
    \newcommand{\dirNewtonptbarrparam}[1][]{\dirNewton[{\pt, \barrparam[]}]}
    \newcommand{\dirNewtonptbarrparamotriter}[1][]{\dirNewton[\ptotriter, \barrparamotriter]}
    \newcommand{\dirNewtonptotriterbarrparamotriterm}[1][]{\dirNewton[\ptotriter, \barrparamotriterm]}
    \newcommand{\dirNewtonptotriterbarrparamotriterp}[1][]{\dirNewton[\ptotriter, \barrparamotriterp]}
    \newcommand{\dirNewtonineqLagmultbarrparam}[1][\ineqidx]{{\dirNewton[{\ineqLagmult[], \barrparam[]}]}_{#1}}
    \newcommand{\dirNewtonineqLagmultbarrparamotriter}[1][\ineqidx]{{\dirNewton[{\ineqLagmultotriter[], \barrparamotriter}]}_{#1}}
    \newcommand{\dirNewtonineqLagmultotriterbarrparamotriterm}[1][\ineqidx]{{\dirNewton[{\ineqLagmultotriter[], \barrparamotriterm}]}_{#1}}
    \newcommand{\dirNewtonineqLagmultotriterbarrparamotriterp}[1][\ineqidx]{{\dirNewton[{\ineqLagmultotriter[], \barrparamotriterp}]}_{#1}}    
    \newcommand{\dirNewtonallvarbarrparam}[1][\ineqidx]{\dirNewton[{\allvar[], \barrparam[]}]}
    \newcommand{\dirNewtonallvarbarrparamotriter}[1][\ineqidx]{\dirNewton[{\allvarotriter, \barrparamotriter}]}
    \newcommand{\dirNewtonallvarbarrparamotriterp}[1][\ineqidx]{\dirNewton[{\allvarotriterp, \barrparamotriterp}]}
    \newcommand{\dirNewtonallvarotriterbarrparamotriterm}[1][\ineqidx]{\dirNewton[{\allvarotriter, \barrparamotriterm}]}
    \newcommand{\dirNewtonallvarotriterbarrparamotriterp}[1][\ineqidx]{\dirNewton[{\allvarotriter, \barrparamotriterp}]}

    \newcommand{\constCauchy}{\kappa_{C}}

    % theoretical analysis
    \newcommand{\tme}{\tau}  % time 
    \newcommand{\tmetwo}{t}  % time for r-LC1,2
    \newcommand{\tmethr}{t}  % time for directional derivative of the merit function
    \newcommand{\tmefour}{t}  % time for Hessian of functions
    \newcommand{\tmefiv}[1][]{t_{#1}}  % time for curves and vector fields along a curve

    \newcommand{\tmesix}[1][]{t_{#1}}  % time for Taylor's theorem for the pullback of the inequality constraints in local convergence

    % well-posedness
    \newcommand{\thldtrradius}[1][\pt]{\delta_{#1}}  % the threshold of the trust region radius
    \newcommand{\constone}[1][]{v_{#1}}  % constant 1
    \newcommand{\deltaone}[2][\pt]{\delta_{#1}^{#2}}  % delta 1
    \newcommand{\thldtrradiustwo}[1][\pt]{\widehat{\trradius[]}_{#1}}  % the 2nd threshold of the trust region radius
    \newcommand{\coeffone}{\alpha}
    \newcommand{\succset}{\mathcal{S}}
    \newcommand{\unsuccset}{\mathcal{P}}
    \newcommand{\inriteridxunsucc}{{\inriteridx}^{\times}}
    \newcommand{\inriteridxsucc}[1][]{\inriteridx_{#1}}

    \newcommand{\ptinriterunsucc}{{\pt[]}^{\inriteridxunsucc}}
    \newcommand{\trslininriterunsucc}[1][]{\trslin_{#1}^{\inriteridxunsucc}}
    \newcommand{\trsquadinriterunsucc}[1][]{\trsquad_{#1}^{\inriteridxunsucc}}
    \newcommand{\allvarinriterunsucc}{{\allvar[]}^{\inriteridxunsucc}}

    % global convergence to KKT points
    \newcommand{\thldtrradiusthr}[1][]{{\delta}_{#1}}  % the 3rd threshold of the trust region radius for assumption on pullbacks of the inequality constraints
    \newcommand{\epsone}{\varepsilon}  % epsilon for assumption on pullbacks of the inequality constraints
    \newcommand{\epstwo}{\delta_{R}}
    \newcommand{\deltatwo}{L_{R}}
    \newcommand{\Lipschitzconstone}[1][]{L^{#1}}  % L-Lipschitz continuity of inequality constraints
    \newcommand{\compactsubset}{\mathcal{Q}}
    \newcommand{\compactsubsettanbd}{\mathcal{T}}
    \newcommand{\thldval}{\tilde{\delta}}
    \newcommand{\length}{\bar{\ell}}
    \newcommand{\pwisecurve}{\gamma}
    \newcommand{\pwisecurveset}[2]{\Gamma_{#1\leftarrow#2}}
    \newcommand{\epsthr}{{\varepsilon^{\prime}}}  % for a proposition on positivity of the pullback of inequality functions
    \newcommand{\deltathr}{\delta^{\prime}}  % for a proposition on positivity of the pullback of inequality functions
    \newcommand{\succsubseqidx}{j}
    \newcommand{\inrsuccsubseqiter}{\inriteridxsucc[\succsubseqidx]}
    \newcommand{\inrsuccsubseqiterp}{\inriteridxsucc[\succsubseqidx+1]}
    \newcommand{\ptinrsuccsubseqiter}{{\pt[]}^{\inrsuccsubseqiter}}
    \newcommand{\ptinrsuccsubseqiterp}{{\pt[]}^{\inrsuccsubseqiterp}}
    \newcommand{\ineqLagmultinrsuccsubseqiter}[1][\ineqidx]{{\ineqLagmult[]}^{\inrsuccsubseqiter}_{#1}}
    \newcommand{\ineqLagmultinrsuccsubseqiterp}[1][\ineqidx]{{\ineqLagmult[]}^{\inrsuccsubseqiter+1}_{#1}}
    \newcommand{\dirinrsuccsubseqiter}{\dir[\ptinrsuccsubseqiter]}  % Should have been dirptinrsuccsubseqiter
    \newcommand{\dirineqLagmultinrsuccsubseqiter}[1][]{\dir[{\ineqLagmult[#1]^{\inrsuccsubseqiter}}]}
    
    \newcommand{\modelfuninrsuccsubseqiter}[1][]{\modelfun[#1]^{\inrsuccsubseqiter}}
    \newcommand{\trslininrsuccsubseqiter}[1][]{\trslin_{#1}^{\inrsuccsubseqiter}}
    \newcommand{\trsquadinrsuccsubseqiter}[1][]{\trsquad_{#1}^{\inrsuccsubseqiter}}
    \newcommand{\trradiusinrsuccsubseqiter}{{\trradius[]}^{\inrsuccsubseqiter}}
    \newcommand{\thldtrradiusfou}{{\trradius[]}^{\prime}}  % the 4th threshold of the trust region radius
    \newcommand{\coefftwo}{\beta}
    \newcommand{\epsfou}{\varepsilon_{g}}  % for a theorem for limit infimum convergence
    \newcommand{\tholdidxone}{K}  % for a theorem for limit infimum convergence
    \newcommand{\epsfiv}{\underaccent{\tilde}{\varepsilon}}  % for a proposition on positivity of the values of inequality functions
    \newcommand{\tholdvaltwo}{\kappa^{H}}
    \newcommand{\coeffthr}{\widehat{\beta}}
    \newcommand{\thldtrradiusfiv}{{\trradius[]}^{\sharp}}  % the 5th threshold of the trust region radius
    \newcommand{\trradiusinritertholdone}{{\trradius[]}^{\tholdidxone}} % trust region radius for the threshold index 1
    \newcommand{\inritertholdoneidx}{\inriteridx_{\tholdidxone}}
    \newcommand{\ptinritertholdone}{{\pt[]}^{\inritertholdoneidx}}
    \newcommand{\trslininritertholdone}[1][]{\trslin_{#1}^{\inritertholdoneidx}}

    \newcommand{\constEigen}[1][]{\kappa_{E}^{#1}}
    \newcommand{\epssix}{\varepsilon}  % for a theorem for limit convergence

    \newcommand{\succsubseqidxtwo}{r}  % used for a contradiction in  a theorem for limit convergence 
    \newcommand{\inriteridxsucctwo}[1][]{\inriteridxsucc[{{\succsubseqidx}_{#1}}]}
    \newcommand{\inrsuccsubseqtwoiter}{\inriteridxsucctwo[\succsubseqidxtwo]}
    \newcommand{\inrsuccsubseqtwoiterp}{\inriteridxsucctwo[\succsubseqidxtwo+1]}
    \newcommand{\ptinrsuccsubseqtwoiter}{{\pt[]}^{\inrsuccsubseqtwoiter}}
    \newcommand{\trslininrsuccsubseqtwoiter}[1][]{\trslin_{#1}^{\inrsuccsubseqtwoiter}}

    \newcommand{\inriteridxsuccthr}[1][]{p_{#1}}
    \newcommand{\inrsuccsubseqthriter}{\inriteridxsuccthr[\succsubseqidxtwo]}
    \newcommand{\ptinrsuccsubseqthriter}{{\pt[]}^{\inrsuccsubseqthriter}}
    \newcommand{\trslininrsuccsubseqthriter}[1][]{\trslin_{#1}^{\inrsuccsubseqthriter}}
    \newcommand{\succprocset}[1][]{\mathcal{R}_{#1}}
    \newcommand{\inriteridxsuccfou}[1][]{q_{#1}}
    \newcommand{\inrsuccsubseqfouiter}{\inriteridxsuccfou}
    \newcommand{\ptinrsuccsubseqfouiter}{{\pt[]}^{\inriteridxsuccfou}}
    \newcommand{\ptinrsuccsubseqfouiterp}{{\pt[]}^{\inriteridxsuccfou+1}}

    \newcommand{\dirptinrsuccsubseqfouiter}{\dir[\ptinrsuccsubseqfouiter]}
    \newcommand{\modelfuninrsuccsubseqfouiter}[1][]{\modelfun[#1]^{\inrsuccsubseqfouiter}}
    \newcommand{\trslininrsuccsubseqfouiter}[1][]{\trslin_{#1}^{\inrsuccsubseqfouiter}}
    \newcommand{\trsquadinrsuccsubseqfouiter}[1][]{\trsquad_{#1}^{\inrsuccsubseqfouiter}}
    \newcommand{\trradiusinrsuccsubseqfouiter}{{\trradius[]}^{\inrsuccsubseqfouiter}}
    \newcommand{\dummyinriteridx}{n}
    \newcommand{\ptdummyinriter}{{\pt[]}^{\dummyinriteridx}}
    \newcommand{\ptdummyinriterp}{{\pt[]}^{\dummyinriteridx+1}}

    \newcommand{\thldtrradiussix}{{{\trradius[]}^{\prime\prime}}}  % the 6th threshold of the trust region radius
    \newcommand{\coefffou}{\gamma}
    \newcommand{\tholdidxtwo}{K^{\prime}}
    \newcommand{\tholdvalthr}{\kappa_{\rm g}}  % bound for gradient of inequality functions
    \newcommand{\tholdvalfou}{\kappa_{\rm H}}  % bound for Hessian of inequality functions
    \newcommand{\tholdvalfiv}{\kappa_{y}}  % bound for Hessian of inequality functions

    \newcommand{\tholdidxthr}{K}
    \newcommand{\trradiusinritertholdthr}{{\trradius[]}^{\tholdidxthr}} % trust region radius for the threshold index 3
    \newcommand{\inritertholdthridx}{\inriteridx_{\tholdidxthr}}
    \newcommand{\mineigvalinritertholdthr}{{\eigval[]}^{\inritertholdthridx}}
    \newcommand{\trsquadinritertholdthr}[1][]{\trsquad_{#1}^{\inritertholdthridx}}

    \newcommand{\epsgradLag}[1][]{\varepsilon_{L}}
    \newcommand{\epssosp}[1][]{\varepsilon_{S}}
    \newcommand{\epscompl}[1][]{\varepsilon_{C}}

    \newcommand{\mineigvalprtl}[1][]{{\eigval[]}^{\min}_{#1}}
    \newcommand{\mineigvalprtlwccone}[1][]{{\eigval[]}^{\min}_{\weakcriticalcone\paren*{#1}}}

    \newcommand{\mineigvalidx}{s}  % used for a theorem of global convergence for the inner algorithm
    \newcommand{\inritermineigvalidx}{{\inriteridx}^{\prime}_{\mineigvalidx}}
    \newcommand{\ptinritermineigval}{{\pt[]}^{\inritermineigvalidx}}
    \newcommand{\dirinritermineigval}{\dir[\ptinritermineigval]}
    \newcommand{\trsquadinritermineigval}[1][]{\trsquad_{#1}^{\inritermineigvalidx}}
    \newcommand{\allvarinritermineigval}{{\allvar[]}^{\inritermineigvalidx}}
    \newcommand{\ineqLagmultinritermineigval}[1][\ineqidx]{{\ineqLagmult[]}^{\inritermineigvalidx}_{#1}}

    % Outer iteration
    \newcommand{\subseqidx}{n}
    \newcommand{\otrsubseqiter}{\otriteridx_{\subseqidx}}
    \newcommand{\otrsubseqiterp}{\otriteridx_{\succsubseqidx+1}}
    \newcommand{\ptotrsubseqiter}{{\pt[\otrsubseqiter]}}
    \newcommand{\ptotrsubseqiterp}{{\pt[\otrsubseqiterp]}}
    \newcommand{\allvarotrsubseqiter}{{\allvar[\otrsubseqiter]}}
    \newcommand{\dirotrsubseqiter}{\dir[\otrsubseqiter]}
    \newcommand{\asymptotactsubset}{\mathcal{W}}

    \newcommand{\consttwo}[1][]{v_{#1}}
    \newcommand{\tholdidxfou}{j^{\prime}}
    \newcommand{\ineqLagmultotrsubseqiter}[1][\ineqidx]{{\ineqLagmult[]}_{\otrsubseqiter #1}}  % k-th Lagrange multipliers for inequality constraints
    \newcommand{\barrparamotrsubseqiterm}{{\barrparam[]}_{\otrsubseqiter - 1}}  % barrier parameter

    \newcommand{\constthr}[1][]{s_{#1}} % Lipschitz-continuity for Hessian 

    \newcommand{\subsetmanitwo}[1][]{\mathcal{N}_{#1}}  % subset for LICQ presearvility 
    \newcommand{\radiusone}[1][]{r}
    % \newcommand{\radiustwo}[1][]{p}
    \newcommand{\vectwo}[1][]{v^{#1}}  % vector 

    \newcommand{\subsetmanithr}[1][]{\mathcal{V}_{#1}}  % subset for LICQ presearvility 2
    \newcommand{\radiustwo}[1][]{r_{#1}}
    \newcommand{\subseqidxtwo}{w}
    \newcommand{\radiustwosubseq}[1][]{\radiustwo[\subseqidxtwo]}

    \newcommand{\idxone}[1][]{\hat{i}_{#1}}
    \newcommand{\vecthr}[1][]{v^{#1}} 

    \newcommand{\wcconebasis}[1][]{e_{#1}}
    \newcommand{\projwcconeaccum}[1][]{\Proj_{\weakcriticalcone}^{\accumsymbol}}
    \newcommand{\idxtwo}[1][]{i}
    \newcommand{\idxthr}[1][]{t}
    \newcommand{\basisone}[1][]{u_{#1}}

    \newcommand{\clipintvl}[1][]{I^{#1}}
    \newcommand{\clipintvlinriter}[1][\ineqidx]{\clipintvl[\inriteridx]_{#1}}
    \newcommand{\clipintvlinritermin}[1][\ineqidx]{\clipintvl[\inriteridx]_{\min #1}}
    \newcommand{\clipintvlinritermax}[1][\ineqidx]{\clipintvl[\inriteridx]_{\max #1}}
    \newcommand{\constfou}[1][]{\underaccent{\tilde}{c}}  % lower bound co
    \newcommand{\constfiv}[1][]{\tilde{c}}
    \newcommand{\vecfou}[1][]{v^{#1}} 

    \newcommand{\ptinriterm}{{\pt[]}^{\inriteridx-1}}  % (l-1)-th point
    \newcommand{\ineqLagmultinriterm}[1][\ineqidx]{{\ineqLagmult[]}^{\inriteridx-1}_{#1}}  % l-th Lagrange multipliers for inequality constraints
    \newcommand{\IneqLagmultmatinriterm}{{\IneqLagmultmat[]}^{\inriteridx-1}}  % (l-1)-th diagonal matrix of Lagrange multipliers for inequality constraints
    \newcommand{\Ineqfuninriterm}{{\Ineqfunmat[]}^{\inriteridx-1}}  % (l-1)-th diagonal matrix of inequality functions
    \newcommand{\dirptinriterm}[1][]{\dir[{\pt[#1]^{\inriteridx-1}}]}
    \newcommand{\dirineqLagmultinriterm}[1][]{\dir[{\ineqLagmult[#1]^{\inriteridx-1}}]^{\rm N}}

    \newcommand{\tholdvalsix}{\kappa_{g}}  % bound for inequality function

    \newcommand{\constsix}[1][]{a_{#1}}  % constant for dist retraction and tanvec norm 
    \newcommand{\tholdvalsev}[1][]{\delta_{#1}}
    \newcommand{\constsev}[1][]{c_{#1}}
    \newcommand{\consteig}[1][]{r_{#1}}

    \newcommand{\closedball}[1][]{B_{#1}}  % open subset on a manifold


    % local convergence
    \newcommand{\constcompllower}[1][]{\underaccent{\tilde}{\varepsilon}_{\rm c}}
    \newcommand{\constcomplupper}[1][]{\tilde{\varepsilon}_{\rm c}}
    \newcommand{\constgradLaglower}[1][]{\underaccent{\tilde}{\varepsilon}_{\mathcal{L}}}
    \newcommand{\constgradLagupper}[1][]{\tilde{\varepsilon}_{\mathcal{L}}}
    \newcommand{\Lipschitzconstthr}[1][]{L_{\rm g}^{#1}}  % L-Lipschitz continuity of the gradient of inequality constraints
    \newcommand{\Lipschitzconstfou}[1][]{L_{\rm H}^{#1}}  % L-Lipschitz continuity of the Hessian of inequality constraints
    \newcommand{\Lipschitzconstfiv}[1][]{\hat{L}_{\rm H}^{#1}}  % L-Lipschitz continuity of the pullback of the Hessian of inequality constraints
    \newcommand{\Lipschitzconstsix}[1][]{\hat{L}_{\rm g}^{#1}}  % L-Lipschitz continuity of the pullback of the Hessian of inequality constraints


    \newcommand{\constnin}[1][]{r}
    \newcommand{\coefffiv}[1][]{c}  % coefficient for barriar parameter update

    \newcommand{\dirptaccum}[1][]{\dir[\ptaccum]}
    \newcommand{\dirineqLagmultaccum}[1][\ineqidx]{\dir[{\ineqLagmultaccum[#1]}]}
    \newcommand{\dirallvaraccum}[1][]{\dir[\allvaraccum]}

    \newcommand{\tholdbarrparamone}{{{\barrparam[]}^{\prime}}}
    \newcommand{\thldtrradiussev}{{{\trradius[]}^{\prime}}}  % the 7th threshold of the trust region radius
    \newcommand{\subsetmanifou}[1][]{\mathcal{P}_{#1}}  % subset for Newton direction
    \newcommand{\constineqLagmultlower}[1][]{\underaccent{\tilde}{v}_{y}}
    \newcommand{\constineqLagmultupper}[1][]{\tilde{v}_{y}}
    \newcommand{\constinactivecompllower}[1][]{\underaccent{\tilde}{v}_{c}}
    \newcommand{\constinactivecomplupper}[1][]{\tilde{v}_{c}}
    \newcommand{\constdirNewton}[1][]{c_{\rm N}}

    \newcommand{\subsetmanifiv}[1][]{\mathcal{P}_{#1}}  % subset for the bound of the Newton direction

    \newcommand{\subsetmanisix}[1][]{\mathcal{P}_{#1}}  % subset for the bound of the Newton direction
    \newcommand{\tholdbarrparamtwo}{{{\barrparam[]}^{\prime}}}
    \newcommand{\tholdvaleig}[1][]{\kappa}

    \newcommand{\subsetmanisev}[1][]{\mathcal{P}_{#1}}  % subset for the bound of the Newton direction
    \newcommand{\tholdvalnin}[1][]{\kappa}
    \newcommand{\tholdbarrparamthr}{{{\barrparam[]}^{\prime}}}

    \newcommand{\tmesev}[1][]{t_{#1}}  % curve of the retraction for key lemma in local convergence analysis

    \newcommand{\numfun}{n}
    \newcommand{\coeffsix}[1][]{a_{#1}}
    \newcommand{\vecsix}[1][]{a_{#1}}
    \newcommand{\vecsixaccum}[1][]{\vecsix[#1]^{\accumsymbol}} 
    \newcommand{\tholdvalten}[1][]{\delta}
    \newcommand{\idxfou}[1][]{t^{#1}}
    \newcommand{\coeffsev}{c}
    \newcommand{\subsetmaninin}[1][]{\mathcal{P}_{#1}}
    \newcommand{\partderiv}[1][]{\partial_{#1}}
    \newcommand{\coordidx}[1][]{i}
    \newcommand{\tmeele}[1][]{t}
    \newcommand{\stdbasis}[1][]{e_{#1}}
    \newcommand{\stdbasists}[1][]{v_{#1}}
    \newcommand{\idxfiv}[1][]{j}
    \newcommand{\idxsix}[1][]{k}
    \newcommand{\idxsev}[1][]{l}
    \newcommand{\diffretrmat}{A}

    \newcommand{\linbarrKKTvecfld}[2][]{\widetilde{\barrKKTvecfld}_{#1}^{#2}}
    \newcommand{\coeffeig}[1][]{{\kappa}_{#1}}

    \newcommand{\inrhesscurvefun}[1][]{h^{#1}}
    \newcommand{\intvlone}{I}
    \newcommand{\vecfldcurvefun}{V}
    \newcommand{\vecfldcurvefuntwo}{S}
    \newcommand{\extvecfldfun}{X}
    \newcommand{\extvecfldfuntwo}{W}
    \newcommand{\constten}[1][]{c_{#1}}
    \newcommand{\constele}[1][]{J}

    \newcommand{\constgradLagNewton}[1][]{c_{\mathcal{L}}}
    \newcommand{\constcomplNewton}[1][]{c_{{\rm c}}}
    \newcommand{\tholdbarrparamfou}{{{\barrparam[]}^{\prime}}}
    \newcommand{\subsetmanieig}[1][]{\mathcal{P}_{#1}}  % subset for the bound of the Newton direction
    \newcommand{\tmeeig}[1][]{t_{#1}} 

    \newcommand{\Debreuconst}[1][]{\tau}
    \newcommand{\consttwe}[1][]{c_{12}}

    \newcommand{\loccoordbarrKKTvecfld}[1][]{F_{#1}}
    \newcommand{\implloccoordbarrKKTvecfld}{\tilde{F}}
    \newcommand{\implvecone}[1][]{\loccoord{l}_{#1}}
    \newcommand{\implvectwo}[1][]{\loccoord{\xi}_{#1}}
    \newcommand{\implconstone}[1][]{\varepsilon}
    \newcommand{\nbhdone}[1][]{\mathcal{N}}
    \newcommand{\vecfiv}[1][]{v_{#1}} 

    \newcommand{\tmenin}[1][]{t_{#1}} 
    \newcommand{\consttht}[1][]{\tilde{c}^{\prime}}
    \newcommand{\constsvt}[1][]{\underaccent{\tilde}{c}^{\prime}}

    \newcommand{\constfot}[1][]{c_{#1}}

    \newcommand{\tmeten}[1][]{t_{#1}} 
    \newcommand{\residone}[1][]{r}
    \newcommand{\constfit}[1][]{c^{#1}_{15}}
    \newcommand{\allvarnonzeroconst}{\dot{\allvar}}
    \newcommand{\constsit}[1][]{\upsilon}

    \newcommand{\nearquadconst}{\gamma}
    
    \newcommand{\Lipschitzconsttwo}[1][]{L_{#1}}  % L-Lipschitz continuity of inequality constraints

    \newcommand{\Cauchypoint}{Cauchy step}
    \newcommand{\eigenstep}{eigenstep}
    \newcommand{\exactsolution}{exact step}

    \newcommand{\hesscomposfun}[1][]{h_{#1}}
    \newcommand{\hesscomposconst}[1][]{\varepsilon_{#1}}

    \newcommand{\subsetmaniten}[1][]{\mathcal{P}_{#1}}  
    \newcommand{\Debreueps}[1][]{\varepsilon}
    
    \newcommand{\asymptoticallyconsistent}{asymptotically consistent}  % asymptotically consistent
    
    % experiment
    \newcommand{\sysdime}{n}
    \newcommand{\J}[1][]{J_{#1}}  % matrix
    \newcommand{\R}[1][]{R_{#1}}  % matrix
    \newcommand{\Q}[1][]{Q_{#1}}  % matrix
    \newcommand{\state}[1][\stateidx]{x_{#1}}
    \newcommand{\stateidx}{j}
    \newcommand{\stateset}[1][]{X^{#1}}
    \newcommand{\obsnum}{N}
    \newcommand{\sampintvl}{h}

    \newcommand{\matrowidx}{i}
    \newcommand{\matcolidx}{j}
    \newcommand{\A}{A}
    \newcommand{\leftconst}[1][\matrowidx\matcolidx]{l_{#1}}
    \newcommand{\rightconst}[1][\matrowidx\matcolidx]{r_{#1}}
    \newcommand{\centerconst}[1][\matrowidx\matcolidx]{c_{#1}}
    \newcommand{\lengthconst}[1][\matrowidx\matcolidx]{k_{#1}}
    \newcommand{\ineqoneboxset}{\mathcal{I}_{1}}
    \newcommand{\ineqtwoboxset}{\mathcal{I}_{2}}
    \newcommand{\Atrue}{\A^{\truesymbol}}
    \newcommand{\truesymbol}{\text{true}}

    \newcommand{\Grassmann}{\text{Gr}}
    \newcommand{\Grassmannian}{Grassmann manifold}
    \newcommand{\matrowdime}{n}
    \newcommand{\matcoldime}{k}
    \newcommand{\vecidx}{m}
    \newcommand{\Rosenbrockcoeff}{\alpha}
    \newcommand{\Rosenbrockcoefftwo}{c}
    \newcommand{\tCG}{tCG}
    \newcommand{\Exact}{exact}
    \newcommand{\typicaldist}{s}


==> latexmkrc <==
#!/usr/bin/perl

$latex = 'platex -synctex=1 %O %S';
$bibtex = 'pbibtex %O %B';
$dvipdf = 'dvipdfmx %O %S';
$pdf_mode = 3;

if ($^O eq 'darwin') {
    $pdf_previewer = 'open -a Preview';
} elsif ($^O eq 'linux') {
    $pdf_previewer = 'evince';
}

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}



# $pdflatex = "
# latexpand old-version/20250120/old_main.tex > old.tex;
# latexpand section/main.tex > new.tex;
# latexdiff old.tex new.tex > diff.tex;
# pdflatex -c %O diff.tex;
# #pdflatex %O new.tex;
# #pdflatex %O old.tex;
# "

# # Uncomment the last two lines if you want the pdfs (via LogsAndOutputFiles) of the latexpanded versions of the old and new main files. (This would take some time).

